Adding Domain Knowledge to Query-Driven Learned Databases

In recent years, \emph{learned cardinality estimation} has emerged as an alternative to traditional query optimization methods: by training machine learning models over observed query performance, learned cardinality estimation techniques can accurately predict query cardinalities and costs -- accounting for skew, correlated predicates, and many other factors that traditional methods struggle to capture. However, query-driven learned cardinality estimators are dependent on sample workloads, requiring vast amounts of labeled queries. Further, we show that state-of-the-art query-driven techniques can make significant and unpredictable errors on queries that are outside the distribution of their training set. We show that these out-of-distribution errors can be mitigated by incorporating the \emph{domain knowledge} used in traditional query optimizers: \emph{constraints} on values and cardinalities (e.g., based on key-foreign-key relationships, range predicates, and more generally on inclusion and functional dependencies). We develop methods for \emph{semi-supervised} query-driven learned query optimization, based on constraints, and we experimentally demonstrate that such techniques can increase a learned query optimizer's accuracy in cardinality estimation, reduce the reliance on massive labeled queries, and improve the robustness of query end-to-end performance.

==> attack.tex <==
%\section{Attacking Learned Query Optimizers via Constraints}\label{section.attack}
%\section{Constraints are Adversarial for Learned Query Optimizers}\label{section.attack}
\section{Statically Identifying Adversarial Queries from a Workload}\label{section.attack}

Naturally, we can retrospectively analyze a query workload to determine where a learning-based optimizer has performed poorly. However, this requires both a trained model and an executed workload.  In this section we propose a method to \emph{statically} identify adversarial queries \emph{a priori}, based on domain knowledge.  As we describe later in this paper, static identification of queries can be useful in \emph{synthesizing new training queries} to improve the learned optimizer's performance.
%
%In this section, we introduce a novel method for attacking learned query optimizers by using database domain knowledge constraints discussed in the previous section. 
Our method is simple, principled, and general which can be applicable to different kinds of constraints. We will empirically demonstrate its effectiveness in Section~\ref{section.evaluation}.% We first define the problem of attacking learned query optimizers.

\medskip

\noindent \textbf{Problem Definition.}
Given a set of $n$ \emph{candidate queries} (which can be training queries or randomly generated queries), we seek to find the top-$k$ \emph{adversarial queries} for which the learned query optimizers are \emph{most likely} to produce bad query execution plans which subsequently lead to slower query running time. For our paper's focus on learned cardinality estimation, our task is to find the \emph{adversarial queries} for which the learned cardinality model will most likely give \emph{bad estimates} that result in a bad query running time performance.% We focus on learned cardinality estimation in this paper.

\subsection{Overall Method} \label{section.attack.steps}
We implement our solution via constraints, which we call a \emph{constraint-based adversarial strategy}. The key idea behind the constraint-based adversarial strategy is \emph{identifying queries with largely underestimated subqueries by the learned cardinality model as the adversarial queries}. The rationale for this idea is intuitive and justified by previous work~\cite{leis2018query, deeds2023safebound,han2021CEbenchmark}: underestimation leads optimizers to produce overly optimistic query plans whose costs are very high for expensive
queries. The proposed constraint attack framework has three steps:
\begin{itemize}  [leftmargin=*]
    \item \emph{Split}: We first split each query into a set of all possible subqueries.

    \item \emph{Pick}: For each query, we pick and keep the subquery with the largest cardinality. For efficiency, here we can use Postgres estimates which are very quick to obtain using the command \texttt{EXPLAIN}. The intuition for \emph{pick} is \emph{if the largest subquery is significantly underestimated and included in the query plan, the query's execution time is more likely to increase.}

    \item \emph{Estimate and Rank}: For all remaining subqueries, we measure the degrees of underestimation by the learned cardinality model using constraints, and then rank them based on the degrees. For the top-$k$ subqueries, we return their \emph{original} queries as the adversarial queries. Here the key issue is how to estimate the degrees of model underestimation via constraints, which we will discuss in the next subsection.

    
\end{itemize}

\subsection{Finding Adversarial Queries via Constraints} \label{section.find-adv}

We then introduce how to use different constraints to estimate the model underestimation degrees for subqueries.


\noindent \textbf{Consistency Constraint.}
Recall that in Section~\ref{subsection.pre.knowledge}, we quantified the cardinality relationship between $q_1$, $q_2$ and $q_3$ if $q_2$ and $q_3$ are split from $q_1$: $c(q_1) = c(q_2) + c(q_3)$. With the equality in mind, for each remaining subquery $q_i$, we randomly choose an unqueried column from all columns involved in $q_i$'s join graph and then sample a \emph{breakpoint} for the chosen column to break $q_i$ into two separated queries $q_{i1}$ and $q_{i2}$.

Afterward, we use the learned cardinality model to estimate the cardinalities for the three queries ($q_i$, $q_{i1}$, and $q_{i2}$).  We measure the model underestimation degrees based on two insights. First, if $\hat{c}(q_i) < \hat c(q_{i1}) + \hat c(q_{i12})$, we know it is a clear violation of consistency constraint for the learned cardinality model. Second, the higher the ratio $\frac {\hat c(q_{i1}) + \hat c(q_{i12})} {\hat{c}(q_i)}$ is, the higher the likelihood of $q_i$ being underestimated by the model, so we call it underestimation ratio. 
As such, we use the underestimation ratio as the predicted underestimation degree to sort all subqueries. Here one may wonder that a higher predicted underestimation degree could be due to $q_{i1}$ and $q_{i2}$ being overestimated, instead of $q_{i}$ being underestimated. In fact, this is the reason why the constraint attack framework chooses the top-$k$ subqueries with the largest underestimation degree --- for a predicted underestimation degree that is sufficiently large, there is a high chance of $q_{i}$ being underestimated even if $q_{i1}$ and $q_{i2}$ are overestimated. We will examine this assumption in Section~\ref{section.evaluation}.






\begin{example} [Measuring the Underestimation Degree by Consistency Constraint] Consider a query $q$ on IMDb which joins two tables \texttt{title}  and \texttt{cast\_info} (\texttt{ci} for short), and $q$ has a predicate: $\{\texttt{ci.role\_id}=10\}$. Then suppose the chosen \emph{breakpoint} column is \texttt{t.year} and the sampled breakpoint is 2000, we obtain two separated queries $q_1$ and $q_2$ with the same join graph as $q$ but split from $q$: $q_1$ has predicates: $\{\texttt{ci.role\_id}=10, \texttt{t.year}<2000\}$; $q_2$ has predicates: $\{\texttt{ci.role\_id}=10, \texttt{t.year}\geq2000\}$. Then, if the learned cardinality model gives estimates 100, 300, and 700 for $q$, $q_1$, and $q_2$, respectively, the predicted underestimation degree is $(300+700)/100 = 10$.

\end{example}

\noindent \textbf{PK-FK Constraint Case 1 - Fact Table holding PK.} This case of PK-FK is applicable to join queries containing PK-FK join and there is no predicate on the fact table with PK. From Section~\ref{subsection.pre.knowledge}, we know that for a query $q$ in this case, $c(q) = c(q_B)$ ($q_B$ is a subquery of $q$ which drops the fact table with PK from $q$). Therefore, for each subquery $q_i$, we drop its fact table to get the subquery $q_{i1}$ of $q_i$.
Then, similar to the consistency constraint, we get their model predictions, $\hat c(q_i)$ and $\hat c(q_{i1})$ and use the ratio $\hat c(q_{i1}) / \hat c(q_i)$ as the predicted underestimation degree. The intuition is likewise to that of consistency constraint --- the higher this ratio is, the more likely $q_i$ is underestimated.




\begin{example} [Measuring the Underestimation Degree by PK-FK Constraint] 
Consider a query $q$ on IMDb which joins two tables \texttt{title} and \texttt{cast\_info} on a PK-FK join, and $q$ has one predicate: $\{\texttt{ci.role\_id}=10\}$. The desired subquery should be query $q_1$ on the table \texttt{cast\_info} with the same predicate as $q$.
Then, if the learned cardinality model gives estimates 100 and 700 for $q$ and $q_1$  respectively, the predicted underestimation degree is $700/100 = 7$.

\end{example}

Astute readers may argue that the use cases of PK-FK constraint are much restricted. However, it is worth noting that the applicable scenario does not compromise the practicality of the PK-FK constraint. First, join queries are much more important than single table queries in query optimization. Second, in fact, in the existing query optimization benchmarks~\cite{}\zi{Fill in} it is common to see queries with no predicate on the fact table. Third, even for those queries having predicates on the fact table, a large fraction of their subqueries contains only FK-FK join. For these subqueries with only FK-FK join, MSCN (and many other learned cardinality methods such as DeepDB~\cite{deepdb}) need to first add the fact table (with no predicate) to them and convert the FK-FK join to multiple PK-FK joins (which will not change the query results), and then estimate the resulting subqueries. The new subqueries precisely meet the applicable criteria of using the PK-FK constraint. Consequently, the PK-FK constraint exhibits broad applicability.


% \noindent \textbf{PK-FK Constraint Case 2 - Fact Table holding FKs.} This case of PK-FK constraint is applicable to join queries containing \emph{multiple} kinds of PK-FK joins and the fact table holding FKs can join with multiple dimensional tables with PK.

==> overview.tex <==
\section{\name: Training Learned Databases with Constraints }

% \subsection{Converting DB Domain Knowledge into Logic Constraints}

% \subsubsection{\textbf{First-Order Logic Framework}}

% First-Order Logic (FOL) is a formal system in mathematical logic that extends Propositional Logic to a more expressive and powerful language capable of representing complex relationships and quantified statements. It consists of 1) \emph{objectives} (queries), 2) \emph{predicates} which represent relationships among objects, 3) \emph{quantifiers} which allows us to make statements about objects, and 4) \emph{functions} which represents operations on objects.  We thus use FOL to represent the relationships among queries and to define constraints which are statements about queries. We define several functions on queries, followed by basic predicates.

% \noindent \textbf{Functions.} 1) $R(q)$  2)  $C(q)$ representing cardinality of $q$ 3) Relational Algebra Operators

% \noindent \textbf{Predicates.} 1) $\text{IsPK}(\text{key})$ 
% 2) $\text{IsFK}(\text{key})$

% \subsubsection{\textbf{Examples}} We formally define the constraints considered in the paper using the first-order logic framework.

% \noindent \textbf{Consistency Constraint.}
% \noindent
% Let $q_1(\bar X), q_2(\bar X), q_3(\bar X)$ be queries over schema $\Sigma$, returning attributes $\bar X$. Then:
% %
% \begin{equation}
%     \begin{aligned}
%         (q_1(\bar X) \cup q_2(\bar X) &= q_3(\bar X)) \land (q_1(\bar X) \cap q_2(\bar X) =  \emptyset) \\
%         & \rightarrow  |q_1(\bar X)| + |q_2(\bar X)| = |q_3(\bar X)|)
%    \end{aligned}
% \end{equation}

% \noindent
% which in fact can also be converted to an approximation:
% %
% \begin{equation}
%     \begin{aligned}
%         (q_1(\bar X) \cup q_2(\bar X) &\approx q_3(\bar X)) \land (q_1(\bar X) \cap q_2(\bar X) \approx \emptyset) \\
%         & \rightarrow  |q_1(\bar X)| + |q_2(\bar X)| \approx |q_3(\bar X)|
%    \end{aligned}
% \end{equation}


% \noindent \textbf{PK-FK Constraint.}
% \noindent
% Let $T$ be a relation in schema $\Sigma$, $q_1, q_2$ be queries over $\Sigma$, and $\bar X \rightarrow T$ be a functional dependency over $\Sigma$. Then:
%
% \begin{equation}
%     \begin{aligned}
%         T(\bar X, \bar Y) & \wedge q_1(\bar X, \bar Z) = q_2(\bar X' \subseteq \bar X \bar Y \bar Z) \land (FD: \bar X \rightarrow T) \\
%        &  \rightarrow  |q_1| \geq |q_2|
%    \end{aligned}
% \end{equation}

% \subsubsection{\textbf{Remark}} One could easily extend the first-order logic framework to include any constraints that can be defined as relationships among queries. 

\subsection{Turning Logical Constraints into Losses} 
To convert logical constraints to losses for which the model can optimize, given a training query, we need to generate relevant queries according to the logical constraints of interest (\S~\ref{section.loss.query}). Then based on the training and generated queries, we define the loss for equality constraints (\S~\ref{section.loss.eq}) and inequality constraints (\S~\ref{section.loss.ieq}).
\subsubsection{\textbf{Constraint-Guided Query Generation}} \label{section.loss.query} 
We first introduce the join schema considered in the paper since as we will see later, there are multiple ways to generate queries for PK-FK constraints depending on the join schema.

\noindent \textbf{Join Schema.} We experiment with two datasets (IMDb~\cite{leis2015good} and DSB~\cite{ding2021dsb}) in the paper. For simplicity, we consider star joins which contain 6 and 5 tables for IMDb (job-light workload) and DSB, respectively. As we will show later, the basic star joins \emph{already} showcase the need for adding domain knowledge to query-driven models and the effectiveness of our framework. We leave more complex join types (\textit{e.g.,} self-join) as future work. As shown in Figure~\ref{fig.join}, for the two datasets, tables are typically joined through PK-FK join. Interestingly, the star join schemas for IMDb and DSB are complementary --- for IMDb, the fact table (\texttt{title t}) having the PK is in the middle and can be joined by other dimension tables with the same key (\texttt{movie\_id}), while for DSB the fact table (\texttt{store\_sales ss}) in the middle holds FKs and joins dimension tables with different keys.

\begin{figure}
\centering
\includegraphics[width=0.47\textwidth]{figs/join-graph}
\vspace{-0.7em}
\caption{Join Schemas for Datasets}\label{fig.join}
\end{figure}


% \noindent \textbf{Applying Consistency Constraint.} We follow the same procedure in Section~\ref{section.find-adv} to generate queries for any training $q$. If there exist feature columns that belong to any table in $q$ and are not queried by $q$, we randomly sample such a column $c$ and then sample a \emph{break point} from the range of $c$ to separate $q$ into $q_1$ and $q_2$. We can subsequently apply the consistency constraint to them.
 
% \begin{example} [Applying Consistency Constraint]
% Consider queries on the table \texttt{title} (\texttt{t} for short) in the IMDb dataset, whose possible queried column is \texttt{t.production\_year} (\texttt{year} for short). Then consider a query $q_1$:$\{\texttt{year}<2000\}$ and two queries split from it: $q_2$:$\{\texttt{year}<1990\}$,  $q_3$:$\{1990\leq \texttt{year}<2000\}$, it is easy to see $c(q_1) = c(q_2) + c(q_3)$.


\noindent \textbf {Applying PK-FK Constraints on IMDb.}. We define two actions \emph{drop} and \emph{add} to generate queries for each training query $q$. Their eligibility is based on the characteristics of $q$:
\begin{itemize}  [leftmargin=*]
    \item  \textit{Drop:} For any $q$ that joins the fact table \texttt{t} with other dimensional tables, if there is some predicate on \texttt{t}, we can \emph{drop} \texttt{t} to get the subquery $q'$ of $q$, which joins dimension tables with FK-FK join. Then we can apply the PK-FK Inequality Constraint: $|q'| \geq |q|$. Moreover, if there is no predicate on \texttt{t}, we use the PK-FK Equality Constraint $|q'|=|q|$, more precisely.

    \item \textit{Add:} Suppose $q$ does not contain the fact table \texttt{t} (\textit{i.e.,} $q$ is a single table query on a dimension table or joins dimensional tables via FK-FK join), we can insert \texttt{t} (no predicate) in the middle of $q$ to be joined with other dimension tables. Then we can apply the PK-FK Equality Constraint to $q$ and the new query $q'$: $|q'|=|q|$.
\end{itemize}



\noindent \textbf {Applying PK-FK Constraints on DSB}. We also define \emph{drop} and \emph{add} on the DSB dataset, which is complementary to that on IMDb. 

\begin{itemize}  [leftmargin=*]
    \item  \textit{Drop:} Suppose in a query $q$, the fact table \texttt{ss} joins some dimensional tables. Then can drop \emph{any} dimension table to get the subquery $q'$ of $q$, to which we can apply the PK-FK Inequality Constraint: $|q'| \geq |q|$. Furthermore, if there is no predicate on the dropped table, we use the PK-FK Equality Constraint $|q'|=|q|$. Note on DSB we choose to drop dimensional tables instead of the fact table as we did on IMDb because according to PK-FK constraints, we can bound the size of the resulting query only by dropping the table with PK.

    \item \textit{Add:} Suppose there exist dimension tables not included in the join graph of query $q$,
     we can join \emph{any} such table (no predicate) with the fact table \texttt{ss}, which forms a new query $q'$. Then we can apply the PK-FK Equality Constraint: $|q'|=|q|$.
\end{itemize}


% \subsubsection{\textbf{Defining Loss for Equality Constraints}}  \label{section.loss.eq}
% it is straightforward to handle equality constraints. Since we already have the label for each training query $q$, we can utilize the label as the ground truth label for the generated query $q'$ (or the sum of multiple generated queries as in the consistency constraint). As a result, we can treat these queries as 'augmented' training queries and define the loss for them in a way similar to the loss for the original training queries. Specifically, we define the Q-error between the generated queries and their labels as the logic loss for equality constraints. One can apply other loss functions such as Mean Square Error, but we empirically observe that Q-error achieves a better performance as it is consistent with the loss function for original training queries.

% In fact, this concept is similar to data augmentation~\cite{shorten2019survey} in the machine learning literature, where a suite of techniques are proposed to generate augmented training data (\textit{e.g.,} images) based on the 'invariant' to a variety of data transformations. The model is then trained on both the augmented data and the original training queries to alleviate over-fitting. Similarly, we propose to leverage the equality constraints as the invariant for query augmentation, \textit{i.e.,} the label (cardinality) should not change after applying equality constraints to generate augmented queries.


% \subsubsection{\textbf{Defining Loss for Inequality Constraints}}  \label{section.loss.ieq}
% We use the notion of \textit{counterexample-guided learning} to define the loss function for inequality constraints. The high-level idea is intuitive ---  1) finding the violations and 2) adding a penalty term to the training loss to correct the violation. The concept of counterexample-guided learning has been applied in the machine learning literature for training monotonicity-constrained neural networks~\cite{sivaraman2020counterexample}.

% However, it is still a non-trivial case compared to equality constraints because we do not have access to the labels for newly generated queries. For example, If we apply the \emph{drop} action to an IMDb query $q$ to get $q'$ and there is some predicate on $\texttt{t}$, then $|q'| \geq |q|$ should hold. By contrast, if the model's prediction for $q'$ is smaller than that for $q$, we are aware that it is a clear violation of the PK-FK constraint. Consequently, we have to include a penalty term in the loss function to correct the violation. However, since there is no ground truth label for the counterexample $q'$, it would be hard to define a logic loss for the model to optimize for.

% \noindent \textbf{First Attempt.} A naive strategy would be directly using the upper bound or lower bound in the inequality constraint to be the ground truth label. Specifically, we can use $|q|$ as the ground truth label for $q'$. Since $|q'| \geq |q|$ and the model predicts $|\hat{q'}| < |\hat{q}|$, we can 'force' the model prediction for $q'$ closer to its real label, but not exactly matching the real value. This is similar to the heuristics used in~\cite{sivaraman2020counterexample} to assign labels (the average of the prediction value for the counterexample and the true label for the training point) to counterexamples. Then we can define the loss as the gap (\textit{e.g.,} Q-error) between $|\hat{q'}|$ and $|q|$ for which we already have the label.





% \subsection{Overview}

% \begin{figure}
% \centering
% \includegraphics[width=0.47\textwidth]{figs/overview}
% \vspace{-0.7em}
% \caption{Overview of \name.}\label{fig.overview}
% \end{figure}

% To address the problems 

% \begin{figure}[!t]
% \centering
% \includegraphics[height=2.9cm]{overview}
% \vspace{-1.8em}
% \caption{Overview of Our Solution
% }\label{fig.overview}
% \vspace{-2em}
% \end{figure}

